Straight Skeletons of Three-Dimensional Polyhedra

This paper studies the straight skeleton of polyhedra in three dimensions. We first address voxel-based polyhedra (polycubes), formed as the union of a collection of cubical (axis-aligned) voxels. We analyze the ways in which the skeleton may intersect each voxel of the polyhedron, and show that the skeleton may be constructed by a simple voxel-sweeping algorithm taking constant time per voxel. In addition, we describe a more complex algorithm for straight skeletons of voxel-based polyhedra, which takes time proportional to the area of the surfaces of the straight skeleton rather than the volume of the polyhedron. We also consider more general polyhedra with axis-parallel edges and faces, and show that any n-vertex polyhedron of this type has a straight skeleton with O(n^2) features. We provide algorithms for constructing the straight skeleton, with running time O(min(n^2 log n, k log^{O(1)} n)) where k is the output complexity. Next, we discuss the straight skeleton of a general nonconvex polyhedron. We show that it has an ambiguity issue, and suggest a consistent method to resolve it. We prove that the straight skeleton of a general polyhedron has a superquadratic complexity in the worst case. Finally, we report on an implementation of a simple algorithm for the general case.

==> complexity.tex <==
\section{Complexity Bounds for Orthogonal Polyhedra}

Most of the skeleton features can be charged to an interaction of two kinds of object: a reflex edge of the original polyhedron boundary, or an edge of a straight skeleton of the polyhedron faces in a single axis-parallel plane. There are n edges of each type, so $O(n^2)$ features.

The exceptional features are those where a face of the wavefront crashes into a larger face moving in the opposite direction, without any two edges of the faces crossing. In this case, one gets a straight skeleton vertex for each corner of the smaller face. However, each vertex of this type is connected by a straight skeleton edge to a vertex not of this type (?), so we can charge these against the other vertices. Collisions of this type can produce convex edges of the wavefront, but not reflex edges. 

\begin{quotation}
\emph{DETAILS TO BE PROVIDED BY DAVID}
\end{quotation}


